A Bregman Method for Structure Learning on Sparse Directed Acyclic Graphs

We develop a Bregman proximal gradient method for structure learning on linear structural causal models. While the problem is non-convex, has high curvature and is in fact NP-hard, Bregman gradient methods allow us to neutralize at least part of the impact of curvature by measuring smoothness against a highly nonlinear kernel. This allows the method to make longer steps and significantly improves convergence. Each iteration requires solving a Bregman proximal step which is convex and efficiently solvable for our particular choice of kernel. We test our method on various synthetic and real data sets.

==> TODO.tex <==
TODO



QUESTIONS 


ANSWERED QUESTIONS

- Do I introduce positive case first and then tackle the negative coefficients problem?
MANON: I lean towards the first option as it seems more natural but it may sound redundant having to write all the problems twice

- We don't really solve the maximum likelihood problem as I got rid of the log\_det term. But maybe we can explain it for the "maximum likelihood" starting point, and argue for better generalisation to other noise distributions. 
